SDR: Efficient Neural Re-ranking using Succinct Document Representation

BERT based ranking models have achieved superior performance on various information retrieval tasks. However, the large number of parameters and complex self-attention operation come at a significant latency overhead. To remedy this, recent works propose late-interaction architectures, which allow pre-computation of intermediate document representations, thus reducing the runtime latency. Nonetheless, having solved the immediate latency issue, these methods now introduce storage costs and network fetching latency, which limits their adoption in real-life production systems. In this work, we propose the Succinct Document Representation (SDR) scheme that computes highly compressed intermediate document representations, mitigating the storage/network issue. Our approach first reduces the dimension of token representations by encoding them using a novel autoencoder architecture that uses the document's textual content in both the encoding and decoding phases. After this token encoding step, we further reduce the size of entire document representations using a modern quantization technique. Extensive evaluations on passage re-reranking on the MSMARCO dataset show that compared to existing approaches using compressed document representations, our method is highly efficient, achieving 4x-11.6x better compression rates for the same ranking quality.

==> bck_evaluation.tex <==
\section{Evaluation}\label{sec:eval}

We start this section by describing the experimental setup (\S~\ref{subsec:exprsetup}), where we introduce the tasks and datasets, and the competing approaches. Next, we present the main results on compression rates and quality tradeoff of the SDR scheme (\S~\ref{subsec:main-evaluation}). Later, we examine how the proposed autoencoder (\S~\ref{subsec:auto-encoder-mrr}) and quantization (\S~\ref{subsec:quantization-evaluation}) compare to other baselines. 
Finally, in \S~\ref{subsec:analysis-vectors}, we provide insights and discuss the information captured by our \oursabbr{}-encoded vectors.

% Building on the evaluation of our method, in this section we aim to provide insights on complementary topics. We start by demonstrating the necessity for this work by evaluating how the document embedding size affects fetching latency (\S~\ref{subsec:analysis-elasticsearch}). Then in \S~\ref{subsec:analysis-vectors}, we discuss on the information captured by our \oursabbr{}-encoded vectors.

\subsection{Experimental Settings} \label{subsec:exprsetup}



\paragraph{\textbf{Tasks and Datasets}} To evaluate the effectiveness of our proposed compression approach SDR and our competing baseline, we consider two tasks from the MSMARCO 2019 Deep Learning Track~\cite{nguyen2016ms}: 

\begin{enumerate}[leftmargin=*]
    \item \textbf{Document Reranking:} In this task, for a given list of top-1000 documents (retrieved via BM25), the task is to rerank the documents such that the most relevant documents for a given query are ranked highest. The performance of models is measured using the mean reciprocal rank, $MRR@10$, metric. This task assess the suitability of the competing approaches in capturing the document context for a given query. We use the development set for this task, which consists of 6980 queries and the corresponding top--1000 documents.
    \item \textbf{Passage Reranking:} Similar as above, here we are given top--1000 passages, and the task is to rerank them such that most relevant passages for a query are ranked highest. This performance of models is measured using the normalized discounted cumulative gain, $nDCG@10$, metric, and assess whether the models can capture the graded passage relevance for a given query. For this task we use the test subset consisting of 200 queries and the corresponding top--1000 passages.
\end{enumerate}

% We use the MSMARCO dataset on the passage re-ranking task~\cite{nguyen2016ms}, which, given a query re-ranks 1000 passages retrieved from BM25.
% In the main evaluation section (\S~\ref{subsec:main-evaluation}) we measure the official MRR@10 metric using the development set, denoted MSMARCO-DEV (6,980 queries). Additionally, for presenting nDCG@10 scores, which require relevance scores for \emph{multiple} documents, we use the TREC 2019 Deep Learning Track test subset \cite{craswell2020overview}, denoted \mbox{MSMARCO-TREC19} (200 queries). In \S~\ref{subsec:auto-encoder-mrr} and \S~\ref{subsec:quantization-evaluation}, where we repeat some of the experiments many times, we reduce the runtime overhead by using a subset of MSMARCO-DEV, denoted \mbox{MSMARCO-DEV-25}, that consists of all queries with only the top 25 results as ranked by a baseline model, which we describe in next paragraph. 

% We denote this subset as \mbox{MSMARCO-DEV-25} and we will describe the baseline model in next paragraph.
% , which . We note that although this is a skewed dataset, in practice it is rare for competitive models to rank in top-10 a document that the baseline ranks below 25.


% The other thing is \cite{craswell2020overview}
% \guy{This is a bit unclear- for each query 25 docs? and than you re-rank only them? If so it might not reflect the actual performance \amit{top-25 ranked by \splitbert. will probably have the same score. we want to prove this if we have the time}}

% \subsubsection*{Task}  We use the passage re-ranking task~\cite{nguyen2016ms}, which ranks 1000 documents per query, and the official metric is MRR@10. \oren{How do you train the model? are you "freezing" the layers? \amit{coming up next...}}
% \amit{@besnik @nachshon, please describe any other task and metric, I've hidden the nDCG related parts for now}

% \amit{for me it seem BM25 should be given some background, or removed}

% The task is to rank the 1000 documents, and the official metric is MRR@10. 

% The entire collection contains 8.8M documents, which can \amit{we?} be used for training the autoencoder network.  \amit{nDCG@10 ??}
% \amit{add MSMARCO 25 here}

% MSMARCO and MASMARCO-DEV-25


\paragraph{\textbf{Baseline -- \emph{\splitbert}}} 
Our algorithm is based on the late-interaction architecture \cite{macavaney2020efficient,gao2020earl,nie2020dc,chen2020dipair,cao2020deformer} depicted in Figure~\ref{fig:late-interaction}. 
We created a model based on this architecture, which we name \splitbert, consisting of 10 layers that are computed independently for the query and the document with an additional two late-interaction layers that are executed jointly. We initialized the model from a BERT checkpoint\footnote{https://huggingface.co/cross-encoder/ms-marco-MiniLM-L-12-v2} with an embedding space of 384 and fine-tuned it using knowledge distillation from an ensemble of BERT-Large, BERT-Base, and ALBERT-Large \cite{hofstatter2020interpretable} on the MSMARCO small training dataset, which consists of almost 40M tuples of query, a relevant document, and an irrelevant document.\footnote{We used a 384 embedding size BERT since this existing checkpoint reached a higher MRR@10 score than a self-trained classical BERT model of standard 768 dimensions. The checkpoint will be released with the published paper.}

\WIP{ 
\nachshon{low priority: Consider https://huggingface.co/cross-encoder/ms-marco-MiniLM-L-2-v2 model. }
}


% \WIP{Since we could not find an existing pre-trained checkpoint, \amit{@nachshon couldn't fine any late interaction checkpoint?, if we describe a training of the latter layers, what was this checkpoint? what was it trained on., etc.,} }
% we implemented the model and initialized it from an existing BERT checkpoint that uses smaller embedding space of 384, but assumes that the query and documents are concatenated from the initial layer. \amit{:prev sentence is a little unclear, what do mean they're concatenated?}
% Then, we run fine-tuning using the MSMARCO small training dataset, which consists of almost 40M tuples of query, a relevant document, and an irrelevant document. 
% Training used knowledge distillation from an ensemble of BERT-Large, BERT-Base, and ALBERT-Large \cite{hofstatter2020interpretable}. 
% 10 layers are computed independently for the query and the document, while the two remaining layers are executed jointly. \amit{prev line should be in the beginning of the paragraph}

% We remark that initial experimentation on 9 independent layers and 3 joint layers and using a BERT with a standard (i.e., 768) embedding size did not have a large impact on the compression capacity.

% That is, even when the embedding size is 768, the compressed vector size remains similar~\footnote{\amit{we already said this in the paragrah:}We used a 384 embedding size BERT since an existing checkpoint reached a higher MRR@10 score than a self-trained classical BERT model of standard 768 dimensions. The checkpoint will be released with the published paper.}.

\paragraph{\textbf{Quantization overhead}}
We incorporate the quantization overhead into the computation of the compression ratios in the following manner: (a) we assume that the additional DRIVE scalar per block (the \mbox{$\ell_2$-norm}) is a float32 and get a space overhead of $32/(\left<\operatorname{block-size}\right>\cdot B)$ where $B$ is the number of bits in the quantization scheme; and (b) we consider the overhead caused by padding, which depends on the length distribution of documents in the dataset. 
For the sake of simplicity, we fixed the block size at 128 and measured the padding overhead using a random sample of 100k documents from the MSMARCO-DEV dataset. This measured padding overhead is
20.1\%,  9.7\%, 6.7\%, and 4.5\%, for \oursabbr 4, 8, 12, and 16, respectively. In \S~\ref{subsec:quantization-evaluation}, we discuss possible means to reduce this overhead.

\paragraph{\textbf{Autoencoder training}}
Although the entire MSMARCO collection contains 8.8M documents, which can be used for training autoencoder networks, in this work we trained autoencoders on a random sample of 500K documents to reduce training time.

\paragraph{\textbf{Notation}}
We denote our SDR variants as ``\mbox{\oursabbr-\{X\}-\{B\}b}'' where \{X\} is replaced with the number of features and \{B\} is replaced with the number of bits in the quantization scheme. When discussing \oursabbr with no quantization we simply write ``\mbox{\oursabbr-\{X\}}''.

\subsection{Main results} \label{subsec:main-evaluation} % \subsection{Experimental Settings} \label{subsec:evaluation-settings} 

% For evaluating the SDR scheme, we use the  MSMARCO-DEV dataset on the passage re-ranking task. Although the entire collection contains 8.8M documents, which can be used for training the autoencoder network, in this work we trained the autoencoder on a random sample of 500K documents to reduce training time.


% \nachshon{I don't see a reason to omit @10 \amit{it's missing in some places, if it's not trivial, we should make sure it's everywhere}}
%We consider the re-ranking task, where for each query, a set of 1000 documents are provided (these are retrieved from the entire corpus using BM25) and the task is to rank these documents such that the relevant ones are at the top of the list. The official metric is MRR@10. For conciseness, we omit the `@10' postfix when the context is obvious. 
%For training a new re-ranking model, MSMARCO provides a training dataset, consisting of almost 40M tuples of query, a relevant document, and an irrelevant document. 
%We report results on the development set, which consists of 6,980 queries and their corresponding 1000 documents per query. 
%The entire collection contains 8.8M documents, which can be used for training the auto-encoder network.
%In this work, we trained the autoencoder networks with a random sample of 500K documents to reduce training time. 



%  \amit{unify with previous section}
% We evaluate the proposed SDR algorithm (\S\ref{sec:algorithm})... \amit{rephrase}


% When using the \Ours{} with X float32 features as ``\mbox{\oursabbr-\{X\}}'', and when adding B bits quantization we use ``\mbox{\oursabbr-\{X\}-\{B\}b}''.
% including the following variants: 
% % \amit{move into one sentence:}
% % \begin{enumerate}
% %     \item \Ours{} with X features (\mbox{\oursabbr-\{X\}}), which applies our autoencoder but no quantization. Storage requirement per document is T*X*4 bytes, where T is the number of tokens in the document. 
% %     % \item DRIVE with B bits (DRIVE-\{B\}), which applies quantization but does not use autoencoder. Storage requirements per document is T*384*X/8 bytes, since the baseline embedding size is 384.
% %     % \nachshon{Why not drive alone? It is still meaningful. \amit{removing since it is not cost effective to explain why the biased version does not work well in this case}}
% %     % \item \splitbert with B bits (\splitbert-\{B\}b), which applies quantization but does not use autoencoder. Storage requirements per document is T*384*B/8 bytes, since the baseline embedding size is 384. \amit{discuss padding overhead and scalar}
% %     \item \Ours{} with X features + B-bits quantization (\oursabbr-\{X\}-\{B\}b), which applies both autoencoder and quantization. 
% %     % Storage requirements per document is T*X*B/8 bytes. \amit{discuss padding overhead and scalar}
% % \end{enumerate}
% Note that ablation study (and alternative schemes) for the autoencoder and quantization parts are discussed in following subsections. 

% AESI-16-NBC-6	nDCG@10=0.772
% AESI-16-NBC-5	nDCG@10=0.772
% AESI-16-NBC-4	nDCG@10=0.766

% AESI-12-NBC-6	nDCG@10=0.780
% AESI-12-NBC-5	nDCG@10=0.778
% AESI-12-NBC-4	nDCG@10=0.764

% AESI-8-NBC-6	nDCG@10=0.775
% AESI-8-NBC-5	nDCG@10=0.770
% AESI-8-NBC-4	nDCG@10=0.765

% AESI-4-NBC-6	nDCG@10=0.766
% AESI-4-NBC-5	nDCG@10=0.767
% AESI-4-NBC-4	nDCG@10=0.752

\begin{table}[]
\setlength{\tabcolsep}{0.3em}
\begin{adjustbox}{center}
	\begin{tabular}{c|c|c|l|l}
	\toprule
		\makecell{Quant. \\ bits ($B$)} & \makecell{\oursabbr \\ dim. ($c$)}      &  \makecell{Comp. \\ ratio (CR)} & \makecell{DEV \\ MRR@10}  & \makecell{TREC19 \\ nDCG@10}   \\
		\hline \hline
 		& \splitbert      & 0.3768                   & 2\\
 		\hline
		\multirow{4}{*}{\makecell{32\\ (float)}}  
% 		0.20\%, 0.0016\%$'$  
		& 16           & 48 & 0.3759 (-$0.20\%$\ignore{, $-0.0042\nicefrac{\%}{\text{CR}}$})     &  0.772 (-$0.2\%$)            \\
		& 12         & 64 & 0.3725 (-$1.14\%$\ignore{, $-0.0178\nicefrac{\%}{\text{CR}}$})$^{*}$       & 0.739 (-$3.5\%$)$^{*}$         \\
		& 8          & 96 & 0.3711 (-$1.51\%$\ignore{, $-0.0157\nicefrac{\%}{\text{CR}}$})$^{*}$ & 0.699 (-$7.5\%$)$^{**}$   \\
		& 4         & 192 & 0.3660 (-$2.87\%$\ignore{, $-0.0149\nicefrac{\%}{\text{CR}}$})$^{**}$        & 0.659 (-$11.5\%$)$^{**}$ \\
		\hline
		\multirow{4}{*}{6}
		& 16 &  243 &  0.3753 (-$0.40\%$\ignore{, $-0.0016\nicefrac{\%}{\text{CR}}$})  & 0.772 (-$0.2\%$) \\
		& 12 & 318 & 0.3728 (-$1.07\%$\ignore{, $-0.0034\nicefrac{\%}{\text{CR}}$})$^{*}$      & 0.780 (+$0.6\%$)  \\
		& 8  & 463 & 0.3689 (-$2.11\%$\ignore{, $-0.0045\nicefrac{\%}{\text{CR}}$})$^{**}$    & 0.775  (+$0.1\%$)   \\
		& 4 & 846 & 0.3624 (-$3.83\%$\ignore{, $-0.0045\nicefrac{\%}{\text{CR}}$})$^{**}$     & 0.766 (-$0.8\%$)   \\
		\hline
		\multirow{4}{*}{5}
		& 16 & 291 & 0.3735 (-$0.87\%$\ignore{, $-0.0030\nicefrac{\%}{\text{CR}}$})$^{*}$           & 0.772  (-$0.2\%$)         \\
		& 12 & 380 & 0.3714 (-$1.43\%$\ignore{, $-0.0038\nicefrac{\%}{\text{CR}}$})$^{*}$        & 0.778  (+$0.4\%$)          \\
		& 8 & 554 & 0.3649 (-$3.16\%$\ignore{, $-0.0057\nicefrac{\%}{\text{CR}}$})$^{**}$       & 0.770  (-$0.4\%$)  \\
		& 4 &  1013 &  0.3540 (-$6.05\%$\ignore{,   $-0.0060\nicefrac{\%}{\text{CR}}$})$^{**}$       & 0.767  (-$0.7\%$) \\
		\hline
        \multirow{4}{*}{4}
        & 16  & 362 & 0.3665 (-$2.74\%$\ignore{, $-0.0076\nicefrac{\%}{\text{CR}}$})$^{**}$       & 0.766 (-$0.8\%$) \\
        & 12   & 472 & 0.3639 (-$3.41\%$\ignore{, $-0.0072\nicefrac{\%}{\text{CR}}$})$^{**}$      & 0.764  (-$1.0\%$)    \\   
        & 8 & 689 & 0.3544 (-$5.95\%$\ignore{, $-0.0086\nicefrac{\%}{\text{CR}}$})$^{**}$           & 0.765 (-$0.9\%$)    \\ 	
        & 4  & 1259 & 0.3408 (-$9.55\%$\ignore{, $-0.0076\nicefrac{\%}{\text{CR}}$})$^{**}$         & 0.752 (-$2.2\%$)$^{*}$ \\  
        \hline \hline
        \multicolumn{2}{c|}{\splitbert (Baseline)} & 2 & 0.3768 & 0.774  \\
		\bottomrule
	\end{tabular}
	\end{adjustbox}
	\caption{MRR@10 and nDCG@10 performance for the different configuration of SDR and the $BERT_{SPLIT}$ baseline over MSMARCO-DEV and MSMARCO-DL19 document and passage re-ranking tasks, respectively. In parentheses for (MRR and nDCG) is shown the absolute difference in percentage points w.r.t the BERT baseline. Using paired t-test statistic we measure statistical significance and denote with $^{*}$ and $^{**}$ significant and highly significant (for $p-value < 0.05$, and $p-value < 0.001$) the results with means different than the baseline. 
	In terms of compression rate reductions, we measured the reduction in contrast to storing the full 768-dimensions from BERT using \texttt{float32} and considering padding and normalization overheads. The highlighted cells are examples of efficient configurations, the first provides 243x compression without a significant lost, and the second provide 1013x compression with only 6.05\% degradation
	\WIP{\nachshon{low priority: consider t-test with margin.}}
	}
	\label{table:main-results}
\end{table}

% \WIP{
% \begin{table}[]
% 	\begin{tabular}{lllc}
% 	\toprule
% 		Algorithm      & \multicolumn{1}{l}{MRR@10} & nDCG@10 &  \multicolumn{1}{l}{Comp. ratio} \\
% 		\hline \hline
% 		\splitbert      & 0.3768    &     0.774                & 2\\
% 		\hline
% 		\oursabbr-4          & 0.3660 (2.87\% $\blacktriangledown$)      & 0.659  (11.5\% $\blacktriangledown$)                     & 192 \\
% 		\oursabbr-8          & 0.3711 (1.51\% $\blacktriangledown$)     & 0.699 (7.5\% $\blacktriangledown$)               & 96 \\
% 		\oursabbr-12         & 0.3725 (1.14\% $\blacktriangledown$)     & 0.739   (3.5\% $\blacktriangledown$)             & 64 \\
% 		\oursabbr-16         & 0.3759 (0.20\% $\blacktriangledown$)     & 0.772 (0.20\% $\blacktriangledown$)                & 48  \\
% 		\hline
% 		\oursabbr-4-6b & 0.3624 (3.83\% $\blacktriangledown$)    &  ?? (??\% $\blacktriangle$)         & 846\\
% 		\oursabbr-8-6b & 0.3689 (2.11\% $\blacktriangledown$)    &  ?? (??\% $\blacktriangle$)         & 463 \\
% 		\oursabbr-12-6b & 0.3728 (1.07\% $\blacktriangledown$)    &  0.780 (0.6\% $\blacktriangle$)                  & 318 \\
% 		\oursabbr-16-6b & 0.3753  (0.40\% $\blacktriangledown$)   &   0.767 (0.7\% $\blacktriangledown$)              & 243 \\
% 				\hline
% 		\oursabbr-4-5b & 0.3540 (6.05\% $\blacktriangledown$)     & ?? (??\% $\blacktriangle$)         & 1013 \\
% 		\oursabbr-8-5b & 0.3649 (3.16\% $\blacktriangledown$)     & ?? (??\% $\blacktriangle$)         & 554 \\
% 		\oursabbr-12-5b & 0.3714 (1.43\% $\blacktriangledown$)     &  0.778 (0.4\% $\blacktriangle$)                & 380 \\
% 		\oursabbr-16-5b & 0.3735 (0.87\% $\blacktriangledown$)     &  0.766 (0.8\% $\blacktriangledown$)                & 291 \\
% 		\hline
% \oursabbr-4-4b & 0.3408 (9.55\% $\blacktriangledown$)    &   ?? (??\% $\blacktriangledown$)            & 1259 \\  
% 		\oursabbr-8-4b & 0.3544 (5.95\% $\blacktriangledown$)    &   ?? (??\% $\blacktriangledown$)            & 689 \\ 		
% 		\oursabbr-12-4b & 0.3639 (3.41\% $\blacktriangledown$)    &   0.764 (1.0\% $\blacktriangledown$)             & 472 \\   
% 		\oursabbr-16-4b & 0.3665 (2.74\% $\blacktriangledown$)    &   0.769 (0.5\% $\blacktriangledown$)               & 362 \\
% 		\bottomrule
% 	\end{tabular}
% 	\caption{\amit{hidden by WIP} Results for different compression techniques. Compression rate is measured compared to storing full 768-dimension BERT vector using the float32 format and considers padding and normalization overheads. MRR@10 drop measures percentage drop compared to the baseline \splitbert model.
% 	\amit{redraw to have $c$ and $B$ as columns}
% 	}
% 	\label{table:main-results-ndcg??}
% \end{table}
% }

The results of SDR evaluation over MSMARCO are reported in Table~\ref{table:main-results}. As can be seen, \ours{} is effective in reducing storage requirements. 
Specifically, \oursabbr-12 reduces storage requirements by 64x compared to a standard 768-dim BERT model, and by 32x compared to a DistilBERT model, with no observable drop in MRR (absolute drop of 0.004). 
\oursabbr-8 show slightly larger drop of 0.006, but reach compression rate of 96x. 
\oursabbr-4 show statistically significant drop of 0.01, which is still minimal, at a storage cost of almost 200x smaller than a naive approach, making it possible to store the entire MSMARCO-DEV dataset in less than 11GB of memory. Finally, the combination of \oursabbr and quantization is highly effective. 
\oursabbr-16-6b reach compression rate of 243x, including padding and normalization overheads, while 
MRR@10 drop is just 0.0015, which is not statistically significant. 
The Average document embedding size is 947 bytes, which, 
as shown in Appendix~\ref{subsec:analysis-elasticsearch}, Table~\ref{table:elasticsearch-latency}, does not significantly increase the fetching latency. 
The entire MSMARCO fits into 8.6GB, which makes it reasonable to store in the RAM of the hosting machine.
If further compression rates are required, \oursabbr-12-4b uses just 6 bytes per token, reaching a compression rate of 472x and 487 bytes per document on average. At this level of compression the entire MSMARCO corpus fits in 4.4GB, making it possible to store it on the GPU memory alongside the model itself. 
The MRR@10 drop is noticeable (0.012), but sill quite low. nDCG@10 results show a similar trend and efficiency although with a bit more noise, which can be attributed to the smaller dataset size.


% DRIVE-B is also an effective strategy for dropping storage requirements, but does not show similar effectiveness to the auto-encoder results. DRIVE-4 provides 8x reduction in storage at \nachshon{Complete once we have numbers. }
%DRIVE-B is also an effective strategy for dropping storage requirements. DRIVE-8 show no loss in MRR. DRIVE-4 reduces storage requirements to 4 bits per float (8x reduction) with very minimal loss in MRR, which is not statistically significant. 
%Even DRIVE-2 drops quality only minimally, but the drop is noticable. 
% \nachshon{Consider returning DRIVE back, then keeping the commented out explanation. Otherwise, we need to rephrase next paragraph.}
% compared to naively storing BERT 
% (i.e., 12 floats with 4 bits per float, or equivalent to 1.5 floats). 

\subsection{Autoencoder Evaluation} \label{subsec:auto-encoder-mrr}
To better understand the impact of the autoencoder, we present MRR@10 results as a function of autoencoder dimension (i.e., number of floats per token that are stored) and with the different variants of autoencoders discussed in \S~\ref{subsec:autoencoder}.

In addition to the 2 dense layer encoder/decoder architecture we described in \S~\ref{subsec:autoencoder} (\textbf{\oursabbr{}-2L}), we consider the following variations:
% \nachshon{@amit to modify format to be similar to 4.4.}
\\\\
\T{AutoEncoder with 2 Layers (AE-2L).} Standard 2-layer autoencoder with $\operatorname{gelu}$ activation. This is the same as AESI only without the side information links. 
	\ignore{\oren{did u tie the weights between the encoder and decoder?
Did u use a normalization layer in the bottleneck in any of the baselines? }}

\T{AutoEncoder with 1 Layer (AE-1L).} Standard autoencoder with a single linear layer in the encoder and decoder.

\T{AESI with 1 Layer (AESI-1L).} \oursabbr{} with a single linear layer in the encoder and decoder with side information links.

\T{DECoder-only AESI (AESI-DEC-2L).} \oursabbr{}, but without providing the side information to the encoder. Recall that the static token embeddings are required by the decoder to help reconstructing the original vector. This variant check if the static token embeddings helps in the encoding part. 
\\
%The uncontextualized token embeddings is mostly important for the decoder, so that the original vector can be reconstructed without relying just on the (few dimension) encoded vector. 
%Therefore, we experiment with an autoencoder where the uncontextualized token embeddings is only provided to the decoder. 
%We further experiment with a single-layer autoencoder with uncontextualized token embeddings, where the 2 layers with a non-linear activation is replaced with a single layer.
%This provides a minor improvement in running time, but is unable to model non-linear combination of the compressed vector with the uncontextualized token embeddings. 


Results are provided in Figure~\ref{fig:auto-encoder-mrr}. 
It can be seen that the side information we provide to the autoencoder (namely, the static token embeddings) is very effective in reducing storage requirements, 
achieving much better MRR@10 when the number of dimensions is small compared to a standard 2-layer autoencoder. 
As expected, a 2-layer encoder/decoder architecture is more effective than a single-layer encoder/decoder. 
The gap is especially large when using static vectors, showing that the interaction between the encoded vector and the static token embeddings is highly nonlinear. 
Finally, we note that it is possible to provide static token embeddings only to the decode, but providing it also to the encoder slightly increase overall MRR@10 score. 
\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{SuccinctDocRepr/figures/mrr_plot.pdf}
    \caption{MRR@10 measured on the MSMARCO-DEV-25 dataset as a function of autoencoder dimensions. The results are shown for standard autoencoders (AE) and our approach (AESI), with single or two layer encoder and decoder networks. The x--axis shows the dimension of the encoded vector $c$. }
    
    % \amit{@besnik, recreate with more descriptive names, also need to have our AESI drawn over the others}}
    \label{fig:auto-encoder-mrr}
\end{figure}


\subsection{Quantization Evaluation} \label{subsec:quantization-evaluation}
\label{sec:altQ}
To study the impact of quantization, we fix \oursabbr{}-16 as our baseline and measure how different quantization strategies and number of bits affect the MRR@10 score. We note that we do not measure quantization over the baseline \splitbert since it can only achieve a compression ratio of up to 32x per coordinate (using 1 bit per coordinate). In addition to {\bf DRIVE} (\S~\ref{subsec:quantization-algorithm}, Algorithm~\ref{code:ourQ}), we consider the following quantization strategies:
\bigskip

\T{Deterministic Rounding (DR) \cite{gershogray92}.}
Maps the input coordinates into the $[0, 2^B-1]$ range using min-max normalization and rounds to the nearest integer.

\T{Stochastic Rounding (SR) \cite{barnes1951electronic, doi:10.1137/20M1334796}.}
Normalizes, as before, using min-max normalization, adds a uniform \emph{dither} noise in $(-0.5, 0.5)$, and then rounds to the nearest integer. This provides an unbiased estimate of each coordinate.

\T{Subtractive Dithering (SD) \cite{1057702, 256489}.}
Same as SR, only now before denormalization, instead of just using the values in \mbox{$\{0,\dots,2^B-1\}$}, we first subtract the original dither noise, which we assume can be regenerated using shared randomness. This is an unbiased estimator with reduced variance.

\T{Hadamard Variants (H-DR, H-SR, and H-SD).}
These variants correspond to the previous methods; only they are preceded by a randomized Hadamard transform.

\T{DRIVE with Bias Correction (DRIVE-BC) \cite[Appendix C.3]{vargaftik2021drive}.}
This variant of DRIVE optimizes for lower bias over the mean squared error (MSE) by multiplying the dequantization result in Algorithm \ref{code:ourQ} by a bias correction scalar: $\norm{x}^2_2/\norm{\hat{y}}^2_2$ .

% \T{Hadamard with Subtractive Dithering (H-SD).}
% Preconditions the input vector using the randomised Hadmard transform before applying SD.


% \T{Hadamard with Stochastic Rounding (H-SR). \amit{todo cite}}
% Preconditions the input vector using the randomised Hadmard transform before applying SR.

% \T{Hadamard with Subtractive Dithering (H-SD).}
% Preconditions the input vector using the randomised Hadmard transform before applying SD.

% \nachshon{Why there is no H-DR?} \amit{never saw it used, but can add for making the story more complete}

% \T{Deterministic DRIVE (D-DRIVE).}
% Same as DRIVE, except we replace the random diagonal matrix with a \emph{constant} \mbox{$D$ with values in $\pm 1$} (sampled once for the entire experiment, where in DRIVE we sample for each \ours).

% \T{Variance-Reduced DRIVE (VR-DRIVE).}
% Same as DRIVE, except (1) After the Hadamard transform, we clip coordinates that are farther than $2\sigma$ from the mean coordinate (where $\sigma$ is the coordinates's standard deviation); and (2) We repeat the process10 times and take the best encoded vector in terms of MSE.
% \\\\

% Normalization is computed over 128-float blocks, which aggregate multiple tokens of a document. 
% If the last block is half filled, we send the entire block (128 floats) if the method uses Hadamard transform, and only relevant coordinates otherwise.

% Since some quantization methods are randomized, we repeat each of them ten times and measure average and standard deviation. 
% For faster evaluation, we use the MSMARCO-DEV-25 subset (\S~\ref{subsec:auto-encoder-mrr}). As described in \S~\ref{subsec:quantization-algorithm}, we quantize over blocks of 128 floats.

\bigskip

We plot the results in Figure~\ref{fig:compress_algo_analysis}. First, we observe that the Hadamard variants perform better than their non-Hadamard counterparts. Second, we see that DRIVE performs better than all other schemes. The differences are more pronounced in the low-bit regime, where the choice of quantization scheme has a drastic impact on quality; when the number of bits is large (e.g., 6), all methods perform reasonably well, and the gap between the quantization schemes is reduced. We also note that unlike in other use cases, such as distributed mean estimation, bias correction is not appropriate here and should not be performed at the cost of increased mean squared error (MSE). This conclusion follows by observing that DRIVE and the deterministic rounding methods (DR, H-DR) are respectively better than DRIVE-BC and the stochastic rounding methods (SR, H-SR). We add that the subtractive dithering methods (SD, H-SD), expectedly, work the same or better than their deterministic counterparts since they produce a similar MSE while also being unbiased.


The current quantization scheme require padding to full 128 blocks. 
For 4-8 \oursabbr{} size, the padding overhead may reach 10\% -- 20\% percent. 
In addition, we send a normalization value per 128-block, which we currently send as a float32 value, adding 4\% -- 5\% additional overhead. 
Padding can be reduced by treating the last 128-block separately, e.g., applying a method that does not require Hadamard transform. 
Normalization overhead can be reduced, e.g., by sending normalization factors as float16 instead of full float32. 
However, such solutions complicate the implementation while providing limited storage benefits, so were not explored in the context of this paper. 
\nachshon{@amir: Add variable length discussion. \amit{and entropy encoding?} }
% TODO: we can obviously see DRIVE works best paragraph (except when it doesn't). See Figure \ref{fig:compress_algo_analysis}.\\
% \amit{things we tried, but probably shouldn't use: repeat, clip}


\begin{figure}
    \centering
    \includegraphics[width=3.2in]{SuccinctDocRepr/figures/mrr_values.pdf}
    % \includegraphics[width=3.2in]{SuccinctDocRepr/figures/compression_mrr.pdf}
    \caption{MRR@10 for different quantization methods. Each run quantize and dequantize \oursabbr{}-16 encoded documents over the MSMARCO-DEV-25 dataset. For each randomized quantization method and number of bits, we take the average of 10 runs. The error bars mark the standard deviation of these runs. 
    
    % \amit{@besnik create with a similar style, but match the existing content, i.e., sixth bit, error-bars, rename DRIVE->DRIVE-BC, rename DRIVE-NBC->DRIVE, remove H\_SR2}
    }
    \label{fig:compress_algo_analysis}
\end{figure}

\subsection{Towards Interpreting \oursabbr{}-Encoded Vectors}
\label{subsec:analysis-vectors}
In \S~\ref{subsec:auto-encoder-mrr}, we showed the effectiveness of our \ours{} over the naive autoencoder architectures by comparing MRR@10 scores for the MSMARCO dataset.
% \amit{removed ", especially when the embedding size is small,", seems irrelevant here}
However, these results incorporate multiple documents and multiple tokens per document, which makes it harder to understand the low-level behavior of \oursabbr{} itself.
In this subsection, we turn our focus to the token level and try to discern when and why adding the static embedding as side information is beneficial.% important, and where the static embedding provide less benefits.
%Our hypothesis is that tokens with a strong standalone meaning would benefit more from static embedding compared to tokens that serve the grammatical structure of the text (e.g., the tokens ``the'', ``a'', or punctuation) and do not have meaning as standalone tokens. 

\paragraph{Intrinsic evaluation for autoencoder}
To study the effectiveness of an autoencoder at the token level (instead of the task level), we propose to use the \emph{reconstruction error}, defined as the MSE between the original vector and the reconstructed vector:
$$MSE(v, D(E(v, u), u)),$$
where $v$ is a contextualized vector (which is the output of a \splitbert{} model at layer $10$), $u$ is the static embedding, and the encoder $E(v, u)$ and the decoder $D(e, u)$ are as defined in \S~\ref{subsec:autoencoder}.
An high reconstruction error imply that the autoencoder had more difficulty in encoding the original vector's information.
% A low reconstruction error indicates that the reconstructed vector is very similar to the original vector, implying low information loss in the compression process. 

\paragraph{Document frequency impact on reconstruction error}
A common result in the area of information retrieval is that the importance of a token is inversely correlated with its frequency. \amit{would be nice if we could cite something here, although this is mostly common sense}
That is, a token appearing in just a few documents is more important for ranking than a token appearing in most documents in the corpus. 
This motivates schemes like TF-IDF, where the importance of a token is affected by the inverse document frequency, as well as the term frequency. 
\\

In Figure~\ref{fig:analysis-idf} we show the reconstruction error as a function of the \emph{Document Frequency} (DF), 
% which we use as proxies for the encoded vectors's information complexity and the token insignificance, respectively.
% DF is 
measured in a logarithmic scale with base 10, that is: $DF(t) = \operatorname{log}_{10}(|\{d \in D:t \in d\}|/|D|)$, where $D$ is the document corpus (this is simply the negation of the standard IDF).
We consider a random sample of 256K documents from MSMARCO, which results in 20M contextualized token embedding. 
Our model uses BERT's tokenizer, with a vocabulary of 30K tokens.
We use a standard 2-layers AutoEncoder with $\operatorname{gelu}$ activation (\textbf{AE-\{X\}}), as well as our \oursabbr (\mbox{\textbf{\oursabbr{}-\{X\}}}).
As in the evaluation section, \{X\} is replaced with the number of features in the encoded vectors. 
We only consider relatively small X values: 1, 2, 4, or 8 floats, since larger sizes have smaller MSE, which makes it harder to identify trends.
\\

First, We observe that given a specific code size, the \oursabbr{} architecture always achieve lower reconstruction error compared to the AE architecture (for all DF values).
This lower reconstruction error correlates with our results in \S~\ref{subsec:auto-encoder-mrr} that \oursabbr{} achieves better ranking quality. Next, we study how the reconstruction error changes with the token frequency. For the autoencoder, there is a slight downward trend in reconstruction error as the frequency increases, which is more pronounced for the most frequent tokens. This can be explained by the fact that more frequent tokens are represented more often in the autoencoder training set, leading to a more accurate representation. 

The gap in reconstruction error between the autoencoder and \oursabbr{} is a way to quantify the effect of adding the static embeddings as side information to the compression process. As seen in the figure, this gap is large for infrequent tokens, and shrinks for frequent tokens. 
% Next, we consider how reconstruction error change with DF. 
% For DF between -6 and -2, the reconstruction error slightly decrease when frequency increases, but the behavior is not stable. 
% Then, for the AE architecture, we see a clear downward trend for DF of -1 and 0, i.e., low reconstruction error for high-frequency tokens. 
% Since tokens' distribution can be viewed as an imbalanced dataset, it is expected that the popular tokens would be represented better (i.e., low reconstruction error).
% For the \oursabbr{} architecture, however, we see the opposite trend, where the reconstruction error {\em increases} for high-frequency tokens.
A possible explanation of this phenomena is that frequent tokens have more meanings, which change according to the context, while lower-frequency tokens often represent words with a single meaning. For example, frequent tokens consist of stop words (e.g., ``the'', ``a'') and punctuation, as well as different suffixes such as ``\#\#ing'' that are a result of the BERT tokenization process. In addition, in the classical work of \citet{britton1978lexical} it was found that frequent words have more distinguished meanings compared to an average word. For tokens with a single meaning, the meaning of the token is already present in its static embedding, so the contextualized embedding can be compressed more aggressively when the static embedding is known. In the other extreme, when a frequent token has many meanings, the contextual embedding can vary greatly, and the static embedding has a more limited effect.

% The standalone meaning of a token is already presented in its static embedding.
% Then, \oursabbr{} can store just how the context changes the standalone meaning of the token. %, which can be done cheaply. 
% In contrast, stop words and punctuation are meaningful only within a context; therefore, the static embedding are less useful for reconstructing the inherently-contextualized representation. 
% Since the reconstruction task is harder for frequent tokens, this explains the observed large reconstruction error for such tokens. 

% For the autoencoder architecture, this phenomena does not happen as it does not receive the static embedding of a word. 
% Since frequent tokens appear more in the data, the network learns to encode such token better, leading to lower reconstruction error for the high-frequency tokens.

% Our results also resonate the classic work of \citet{britton1978lexical}, who found that frequent words have more distinguished meanings compared to an average word. 
% If \oursabbr{} encodes the specific meaning of a word within a context, it becomes more difficult where the number of meanings is larger, which can also explain the phenomena observed in Figure~\ref{fig:analysis-idf}. 


%---------------
%\amit{(TODO) make this sound less generic, less about the context meaning, maybe change the title}
%
%
%After showing the effectiveness of the \ours architecture, we now attempt to have an in-depth understanding on how the static token embeddings help. 
%Specifically, we hypothesize that \ours{} can store only the ``context'' of a word, while a standard autoencoder has to store the entire meaning of the word. 
%We therefore expect a higher error rate for \ours{} when the context is highly important, and a smaller error rate otherwise. 
%
%To test this hypothesis, we start by selecting a random sample of 256K documents. 
%Each autoencoder variant is run on these documents, generating pairs of 
%original vector (uncompressed token embedding) and reconstructed vector (after the encoding and decoding, without quantization). 
%We then denote by {\em reconstruction error} the mean square error (MSE) rate between these two vectors. 
%We consider this as a measure for the difficulty of encoding a token - with lower MSE (at a given compressed dimension) implying a token that is ``easier'' to encode. 
%
%
%\paragraph{Studied autoencoders} We consider a standard 2-layers AutoEncoder and $\operatorname{gelu}$ activation (\textbf{AE-\{X\}}), as well as our \oursabbr (\mbox{\textbf{\oursabbr{}-\{X\}}}). As in the evaluation section, \{X\} is replaced with the number of features in the encoded vectors. We only consider relatively small X values: 1, 2, 4, or 8 floats, since larger sizes have smaller MSE, which makes it harder to identify trends.
%
%
%\paragraph{Document frequency impact on reconstruction error}
%A common result in the area of information retrieval is that the importance of a token is inversely correlated with its frequency.
%That is, a token appearing in just a few documents is more important for ranking than a token appearing in most documents in the corpus. 
%This motivates schemes like TF-IDF, where the importance of a token is affected by the inverse document frequency, as well as the term frequency. For out purpose, we try to see if we can spot a trend between the document frequency, as an inverse measure of importance, and the reconstruction error. We use document frequency in base-10 log, defines as: $DF(t) = \operatorname{log}_{10}(|\{d \in D:t \in d\}|/|D|)$, where $D$ is the document corpus (this is just the negation of the standard IDF).\\
%
%\WIP{
%Note that we expect frequent terms to have better reconstruction error, since the autoencoder is exposed to many more such tokens, and therefore can specialize for them. \guy{I'm not sure about this last sentence. Since you try to learn only the context (at least for some of the encoders in question), isn't what's important the frequency of the context and not the frequency of the token?}}
%
%% We common measure $\operatorname{IDF}$ reconstruction error as a function of minus inverse document frequency with log base 10, defined as:
%% $$-IDF(t) = -\log_{10}(N/\mbox{\em DocumentFrequency}(t))$$
%% We multiplied IDF by -1, so that $10^{X}$ is the frequency of the token with $IDF(t)=X$ (e.g., -2 implies the token appears in 0.01 of all documents). 
%
%Results are depicted in Figure~\ref{fig:analysis-idf}. For DF between -6 and -2, the reconstruction error slightly decrease when frequency increases. 
%For the AE, the trend continuous and intensify for DF of -1 and 0. Such tokens are frequent, so the autoencoder specializes in reconstructing them well. 
%For the \oursabbr{}, in contrast, the trend is reversed, and the reconstruction error is much higher for high-frequency tokens. \guy{this is what I meant in my last comment, so I guess your expectation was just for the standard encoders? maybe emphasize this?}
%High-frequency tokens are also denoted as stop words (e.g., the word ``the''), \guy{note this can also be word pieces or even letters, numbers, punctuation etc. Same intuition is still relevant because all of these obviously rely much on the context, but still maybe worth noting.}
%for which the meaning heavility depends on the context. 
%Therefore, the static token embedding is less useful for reconstructing the contextualized meaning of this token. 
%Of course, such tokens are less useful for ranking, so a higher reconstruction rate for such tokens is less likely to impact overall ranking quality. 
%\amit{there is an hidden assumption that frequent words depend more on context, this is a bit hand-wavy, and maybe its better to emphasis that this is just a just suggested conjecture/our intuition from relating to this experiment.}
%\guy{re Amit's comment: The fact that frequent words have more meanings (and therefore "depend more on context") is pretty known. For example  \hyperlink{https://link.springer.com/article/10.3758/BF03205079}{here} (yes it's old, like all main linguistic work) it is shown that out of the 100 most common words in English, 93\% have more than one meaning while in the rest of the language it's about 30\%. Having said that, and relating to my last comment, here we are talking about the most common TOKENS and not words, and this might behave differently, since the uncommon words are splited to sub words and saying something about the distribution of tokens is harder + tokenizer dependent.}

\begin{figure}
	\centering
	\includegraphics[width=1.0\columnwidth]{SuccinctDocRepr/figures/mse_reconstruction_error_idf.pdf}
	\caption{Reconstruction Error vs. DF for the different \mbox{AE} and \mbox{AESI} configurations. Our approach, AESI, is very robust in recovering back the token's representation with a minimal reconstruction error rate (y-axis), which is constant for documents with varying DF scores. It is interesting to note that for frequent tokens (i.e., tokens that are function words, hence play a marginal role in retrieval), the error rate is higher when compared to the rest of the tokens.\amit{todo explain smoothing window / averaging}}
	
% 	We plot AutoEncoder (AE) and the \oursabbr{} models with filled and empty markers, respectively. }
	
% 	\amit{@besnik changed the caption for now, we need to recreate the graph or change the previous sentences: "Reconstruction error rate vs. inverse document frequency. In black (and triangle markers) we plot autoencoder models. In blue (and circle markers) we plot \oursabbr{} models Different shades imply different number of encoded dimension." (also note it says AEU in the graph)} }
	\label{fig:analysis-idf}
\end{figure}

%Finally, we note that even for high-frequency tokens, the reconstruction error rate is always better for \ours{} compared to a standard autoencoder. 
%This demonstrates that the system still uses the token information for better encoding. \oren{Not convinced. Is there some references that the high-frequency words "require" more context?
%
%Just an idea... what about using the variance of the final token embedding as the "contextual" proxy instead of the frequency?}
%

